A Graphical Language for Real-Time Critical Robot Commands

Industrial robotics is characterized by sophisticated mechanical components and highly-developed real-time control algorithms. However, the efficient use of robotic systems is very much limited by existing proprietary programming methods. In the research project SoftRobot, a software architecture was developed that enables the programming of complex real-time critical robot tasks with an object-oriented general purpose language. On top of this architecture, a graphical language was developed to ease the specification of complex robot commands, which can then be used as part of robot application workflows. This paper gives an overview about the design and implementation of this graphical language and illustrates its usefulness with some examples.

==> sec.rapicommands.tex <==
\section{The Robotics API Command Model (\textit{TODO:Lehrstuhl})}
\label{sec:rapicommands}

Robot tasks (with real-time requirements) in the Robotics API are expressed as \textit{commands} (cf. Fig.~\ref{fig:commands}). Such commands abstract from the concrete job performed, and provide a common interface.
A robot task consisting of an action for an actuator is encapsulated as a \textit{runtime command}. When multiple (runtime) commands are to be executed with given timing requirements, they can be composed into \textit{transaction commands}. Each transaction command contains a set of initial commands (optionally with start conditions) that will  be executed once the transaction command starts (if the corresponding start condition holds), and a set of further commands that can be executed later based on events.

\begin{figure}[htbp]
	\centering
		\includegraphics[width=0.85\linewidth]{images/Commands}
	\caption{Commands in the Robotics API}
	\label{fig:commands}
\end{figure}

In the context of a command, \textit{event handlers} can be defined. These monitor when a certain state (action, device, sensor, composed or command state) is entered, and perform one of the pre-defined effects. For runtime commands, the following \textit{effects}\footnote{Additionally, the effect \textit{Takeover} is available, requesting a command to exit as soon as appropriate, leaving the actuator in a consistent, but not necessarily stable state. A command may then assume that the following command will immediately take the actuator in the current situation (and maybe motion) and continue operation. For industrial robots, this can be used to change the executed task without requiring the robot to stop during the task switch (e.g. blending motions). From an implementation point of view, Takeover is similar to Cancel, so further details are omitted here.} are allowed:

\begin{itemize}
  \item \textit{Stop} forcefully stops the execution of the command, without giving the action or device any chance to clean up or perform any further steps. 
  \item \textit{Cancel} asks the command to bring the actuator into a secure, stable state and afterwards exit the command. This state may not require any action to be executed immediately. For a robot motion, Cancel should brake the robot until halt, and then terminate the command.
  \item \textit{Raise} activates another state (that can be handled in further event handlers).
  \item \textit{External} effects notify the non-realtime application that the event has occured. Possible results are starting a Robotics API thread or throwing an exception to allow non-realtime error handling.
\end{itemize}

Due to their structure, transaction commands additionally allow the event effect \textit{Start}, starting a child command of the transaction. Furthermore, \textit{Stop} and \textit{Cancel} may there be applied to the transaction command itself as well as to any of the child commands. However, stopping another command does not give it time to clean up and can lead to unexpected consequences, thus it should only be used in extreme cases. Instead, cancel or takeover are preferred. Stopping a transaction command immediately stops all child commands, but for cancel requests the transaction command has to decide how to handle them (e.g.~by forwarding them to one or some of its child commands).

Besides RuntimeCommands and TransactionCommands, a third command type is available: \textit{Wait commands} remain active for the given wait period (unless cancelled), and can be used to describe defined time intervals between the execution of certain steps. Additionally, by adding event handlers they can also be used to wait for sensor events. WaitCommands can e.g. be used when controlling devices connected via field bus. Here, it can be necessary to set one value, and then wait for a given amount of time and reset the value.

Transaction commands are also allowed to contain further transaction commands as children, so complex command structures can be built, e.g. for combining typical coordination patterns such as parallel and sequential execution.


==> sec.rapiconcepts.tex <==
\section{Basic Robotics API Concepts (\textit{TODO:Lehrstuhl})}
\label{sec:rapiconcepts}

When describing robot activities in the Robotics API, the activity is split into an \textit{action} and the corresponding \textit{actuator}.  

An \textit{action} is a description of what to do, independent from the concrete actuator instance that will execute it. Semantically, actions can be separated by the type of actuator they can be applied to, e.g. into tool actions (such as open and close for a gripper) or motions (such as linear, spline or point-to-point motions). From a behavioural point of view, they can be categorized into goal actions (that specify a goal the actuator shall reach anytime in the future) and step actions (that specify values to immediately apply to the actuator). Examples for goal actions are asking a mobile robot to go to a certain position in space (maybe avoiding obstacles on the way), or opening or closing a parallel gripper. Step actions describe trajectories (telling the robot where to be at every time instant), or other processes where the exact path taken matters for the success of the execution. 

The \textit{actuator} (as a specialization of a \textit{device}) describes and represents a controllable physical object. Note that actuators in the Robotics API (as well as sensors and actions) do not contain implementations for the real hardware (actuators and sensors) or the task execution (actions), but only represent certain code present in the Robot Control Core that will control the described actuator or perform the corresponding task. Hence, the Robotics API objects can be seen as proxy objects for the real-time capable driver implementations on the Robot Control Core. 


\begin{figure}[thbp]
	\centering
		\includegraphics[width=0.85\linewidth]{images/RAPI}
	\caption{Basic Concepts in the Robotics API}
	\label{fig:rapi}
\end{figure}

Additionally, \textit{states} and \textit{sensors} (cf. Fig.~\ref{fig:rapi}) can be used in task descriptions. 
\textit{Sensors} represent values that are available (and can change) during the execution of robot tasks. They can be provided by ``typical'' sensor devices, such as laser rangefinders, light barriers, or field bus inputs, as well as by actuators which provide their state (joint angles, Cartesian position). Other sensors might represent values that can be controlled from non-realtime Robotics API applications (in cases where no exact timing is required). Furthermore, sensor values can be the result of real-time calculations working on other sensor values. Sensors values can be used in actions, e.g. to describe sensor guided motions, and provide states.

\textit{States} represent certain Boolean conditions of sensors, actions or actuators: \textit{Sensor states} are either Boolean-value sensors (where the sensor value ``true'' means that the state is active), or conditions defined on sensor values of other data types. Typical sensor states might be a digital input being on or off, a force sensor exceeding a specified force limit or the fact that an obstacle has been detected by a laser range finder. \textit{Action states} describe certain progress properties of an action. Examples are states telling that a certain via-point of a trajectory has been passed, or that the action has started or completed (i.e. the last set-point has been produced). \textit{Actuator states} include certain error states of the device (e.g. that the commanded set-point is invalid or that an emergency stop has occured), and a completion state (whenever the actuator has reached its latest set-point). Based on these basic states, \textit{composed states} can be defined, e.g. when another state is not active, when two states are active at the same time, or when another state has ever been active. 

